A Homotopy Method for Large-Scale Multi-Objective Optimization

A homotopy method for multi-objective optimization that produces uniformly sampled Pareto fronts by construction is presented. While the algorithm is general, of particular interest is application to simulation-based engineering optimization problems where economy of function evaluations, smoothness of result, and time-to-solution are critical. The presented algorithm achieves an order of magnitude improvement over other geometrically motivated methods, like Normal Boundary Intersection and Normal Constraint, with respect to solution evenness for similar computational expense. Furthermore, the resulting uniformity of solutions extends even to more difficult problems, such as those appearing in common Evolutionary Algorithm test cases.

==> Application.tex <==
%As simulation forms the third scientific pillar, next to theory and experiment,
%simulation-based optimization 

The design and operation of particle accelerators requires balancing a multitude
of control inputs to optimize any number of desired output parameters.  For
instance, when discussing optimial beam dynamics, we aim to minimize the beam
dispersion in both position space, $RMS_x$, and momentum space, $RMS_s$.  Given
the control parameters allowed, $\sigma_x$ and $V_acc$, this unfortunately
involves a trade-off between objectives as they can not be simultaneously
minimized.  Therefore, we aim to sample the Pareto front spanning these
conflicting design criteria.  We will leverage the Object Oriented Parallel
Accelerator Library, OPAL \cite{Adelmann2009}, to simulate the charged particle
optics.

The result is a simple bi-objective optimization problem with two independent
variables.  The real complexity of this problem lies in the fact that, while
considerable effort has been spent on reducing the cost of simulating the beam
dynamics through parallelization \cite{Ineichen2012} and other adaptive
techniques, the forward solver mapping the design variables to the objective
space remains computationally expensive.  Therefore, we will seek to reduce the
number of required forward solves as much as possible.  

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.5]{rms_s_close.png}
  \captionof{figure}{RBFN surrogate function trained with data (shown as dots)
  obtained by running OPAL-based forward solves on a regular set of design
  variables.  Note the fidelity and smoothness of the interpolation.}
  \label{graph:rms_s}
\end{figure}

First, as in \cite{Alonso2009}, we run a set of simulations (in our case,
approximately 330) corresponding to a grid in the design space.  We then
construct a Radial Basis Function Network (RBFN) surrogate \cite{Queipo2005}
using these simulations.

After building an RBFN interpolation for each output variable, we applied
algorithm \ref{alg:Homotopy} to the resulting bi-objective problem.  Figure
\ref{graph:example} illustrates the obtained discrete Pareto front
representation.

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.5]{example.png}
  \captionof{figure}{Pareto front consisting of 120 points and showing the
  trade-off between minimizing $RMS_s$ and $RMS_x$.  The point colors indicate mesh-subset membership or the
  processor with which each sample was obtained.  This particular result was
  computed across 8 different minimization processes running on the Brutus
  cluster at ETHZ.}
  \label{graph:example}
\end{figure}

To demonstrate the strong scalability of our approach, we repeated the
same calculation while varying the processor count.  We performed the following
experiments on the Brutus cluster at ETH Z\"{u}rich.  The cluster consists of
1008 nodes totalling 19,760 processing cores connected by an InfiniBand QDR
network and attains a throughput of over 200 teraflops.  The main program was
compiled with GCC 4.6.2 and executed with the use of the MPICH runtime.  The
current policy of the Brutus standard queue system allows only 128 cores to be
used simultaneously per job.  Since the opt-pilot framework maps each
process type (Optimizers, Pilots, and Workers) to a different core, each
optimization instance really requires three processors.  Therefore, the maximum
number of simultaneous optimization instances we are able to run in this
configuration is 42.  The asynchronous message exchange between processors
introduces a small bit of non-determinism and therefore scatter in our data,
which was mitigated performing five runs and averaging the results, reported in
table \ref{tab:strong}.

Figure \ref{graph:strong} represents the speedup results in graphical form and
compares them to perfect strong scalability.  We were limited in our scalability
tests by the alloted core limits on the Brutus cluster.  However, since
we only computed 120 sample points, the roll-off at the end of the range may
be attributable to poor load balancing.  In our case, some processors will only
have two points to optimize, while others have three, resulting in a 50\%
overload.

\bigskip
\begin{minipage}{\linewidth}
\centering
\captionof{table}{Strong Scalability} \label{tab:strong} 
\begin{tabularx}{\linewidth}{@{} C{1in} C{.85in} *4X @{}}\toprule[1.5pt]
\bf Processor Count  & \bf Time (s) & \bf Speedup \\
 \midrule	1	&	1529.05	&	1		\\
 \midrule	2	&	916.831	&	1.995	\\
 \midrule	4	&	527.761	&	3.718	\\
 \midrule	8	&	318.502	&	7.223	\\
 \midrule	16	&	145.563	&	15.13	\\
 \midrule	32	&	84.524	&	29.36	\\
 \midrule	42	&	70.9816	&	39.94	\\
\bottomrule[1.25pt]
\end {tabularx}\par
\bigskip
Wall-clock time-to-solution for method \ref{alg:Homotopy} on a bi-objective
surrogate-based problem averaged over 5 runs on the ETHZ Brutus cluster.
\bigskip
\end{minipage}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.5]{scalability.png}
  \captionof{figure}{The strong scalability of our Pareto front sampling
  approach (red dots) as compared with a perfect linear speed up (solid line).
  The extent of our scaling test was limited by the standard core allowances on the Brutus cluster.}
  \label{graph:strong}
\end{figure}



